Task-oriented Communication Design in Cyber-Physical Systems: A Survey on Theory and Applications

Communications system design has been traditionally guided by task-agnostic principles, which aim at efficiently transmitting as many correct bits as possible through a given channel. However, in the era of cyber-physical systems, the effectiveness of communications is not dictated simply by the bit rate, but most importantly by the efficient completion of the task in hand, e.g., controlling remotely a robot, automating a production line or collaboratively sensing through a drone swarm. In parallel, it is projected that by 2023, half of the worldwide network connections will be among machines rather than humans. In this context, it is crucial to establish a new paradigm for designing communications strategies for multi-agent cyber-physical systems. This is a daunting task, since it requires a combination of principles from information, communication, control theories and computer science in order to formalize a general framework for task-oriented communication design. In this direction, this paper reviews and structures the relevant theoretical work across a wide range of scientific communities. Subsequently, it proposes a general conceptual framework for task-oriented communication design, along with its specializations according to the targeted use case. Furthermore, it provides a survey of relevant contributions in dominant applications, such as industrial internet of things, multi-UAV systems, tactile internet, autonomous vehicles, distributed learning systems, smart manufacturing plants and 5G and beyond self-organizing networks. Finally, it highlights the most important open research topics from both the theoretical framework and application points of view.

==> Application_OTA.tex <==
%\todoQL{Add an application in network level optimization in 5G/6G.}

%\QL{We may add a subsection of Over-The-Air (OTA) Computation which lies in the intersection of information theory and communication theory. This is a hot topic in communications community that takes into account the underlying task, such as computing a function, directly at the physical layer, by exploit the superposition property of the wireless channel. It allows an efficient function computation over the “air”. Here you may consider the pre-processing of the information as the \lq\lq coding policy", and the post-processing to the final desired function directly as the "action policy". References: \cite{liu2020over,cao2020optimized, frey2020over}} 

\subsection{Over-The-Air Computation in Smart Manufacturing Plants} \label{subsec:AirComp}
In IoT networks, massive amounts of data are generated, collected, and leveraged to help complete a predefined task. For example, in smart manufacturing plants, wireless data needs to be collected from thousands of sensors. However, we are not interested in the value of each individual data source, instead, we aim to obtain the \lq\lq fusion\rq\rq \ of the information contained in all data sources, e.g., computing sums or arithmetic averages. On one hand, transferring raw measurements from a large amount of different data sources to the same data collector is not spectrum efficient, especially when the measurements can be encoded to small data packets. On the other hand, the computation of massive data in an edge device as data collector with limited computation capacity can be also challenging. 

Therefore, the technique called over-the-air computation (AirComp) has been developed to enable communication- and computation-efficient data fusion of the sensing data from large amount of the concurrent sensor transmissions. It takes into account the underlying task, such as computing a function, directly at the physical layer, by exploit the superposition property of the wireless channel. In other words, it allows an efficient target function computation over the \lq\lq air\rq\rq. 

The AirComp is defined as follows. Consider $K$ wireless sensors, each having a measurement signal $s_k\in\R$, $k\in\Ks:=\{1, \ldots, K\}$ to send. On the receiver side, we expect to derive the function of the measurements of the form 
\begin{equation}
    f(s_1, \ldots, s_k) = F\left(\sum_{k=1}^K f_k(s_k)\right)
    \label{eqn:OTA_fkn}
\end{equation}

Given the multiple access communication channel $h:\field{C}^K\to\field{C}$, AirComp aims at finding a set of \textbf{pre-processing functions} $\zeta_k:\R\to\field{C}$ and a \textbf{post-processing function} $\psi:\field{C}\to \R$ such that 
\begin{equation}
f(s_1, \ldots, s_k) = \psi\Big(h\big(\zeta_1(s_1) \ldots, \zeta_K(s_K)\big)\Big)
    \label{eqn:OTA_obj}
\end{equation}
%
The pre-processing of the measurement signal and the post-processing of the received channel output obtain directly the desired computation of the target function in \eqref{eqn:OTA_fkn} by effectively integrating the communication and the computation policies. Moreover, in this way the receiver's computational task $f(\cdot)$ defined in \eqref{eqn:OTA_fkn} of processing $K$ signals is decomposed into $K+1$ small tasks $\left\{\zeta_1(\cdot), \ldots, \zeta_K(\cdot), \psi(\cdot)\right\}$ that can be distributed among sensors and the receiver, with each of them processing only one signal. 

Without loss of generality, AirComp also falls into the class of TOCC. The task is to compute $f(s_1, \ldots, s_k)$ at the receiver (e.g., a center unit) side. The problem defined above can be aligned with Definition \ref{def:TOCC} by simply integrating the computing policy into the communication policy, i.e., the encoding (pre-processing) and decoding (post-processing) policies included in the communication policy already provide the direct action to compute the desired target function as shown in Fig. \ref{fig:OTA}.  

   \begin{figure}[t]
          \centering
              \includegraphics[width=\columnwidth]{OTA.pdf}
          \caption{Over-the-air computation in smart manufacturing plants aligned with the task-oriented communication system design}
          \label{fig:OTA}
    \end{figure}

The authors of \cite{liu2020over} derived theoretical bounds on the mean squared error for a certain AirComp function (sum of the signals) computation in a fast-fading scenario with Channel State Information (CSI) available at the transmitter.  In \cite{dong2020blind}, the AirComp problem is tackled without the explicit knowledge of channel information but under the assumption of slow fading.  Then, in \cite{frey2020over} a AirComp scheme was proposed for distribution approximation of a larger class of functions than the previous works with theoretically proven bound over fast-fading channels that can deal with correlated fading and requires no CSI.

A popular application of AirComp computational techniques is the computation of distributed gradient descent to solve the empirical risk minimization problem for machine learning models. One example is the training of neural networks in a central mode but with distributed data reported by a large number of local agents such as sensors in the smart manufacturing plant. In \cite{amiri2020machine} the authors proposed to use AirComp computation over wireless channels to help efficiently computing distributed stochastic gradient descent in the Federated Learning (FL) paradigm. The author in \cite{yang2020federated} extended the idea to channels with fading channel information at either the transmitter or receiver side. In \cite{frey2020over} the authors shown the application of a proposed AirComp scheme to the regressor and classifiers in vertical FL.


\subsection{5G Self-Organizing Networks}\label{subsec:5GSON}
Although it has been almost a decade since the concept of Self-Organizing Networks (SONs) was introduced to the Next Generation Mobile Networks (NGMN) and 3GPP standards \cite{TS32500}, the existing SON solutions have not met the high expectation of the operators to achieve a fully self-aware cognitive network with automated configuring, monitoring, troubleshooting, and optimizing. This is because, with the emergence of new wireless devices and applications, it is expected that a large amount of measurements and signaling overhead will be generated in future networks, while partial and inaccurate network knowledge, together with the increasing complexity of envisioned wireless networks, pose one of the biggest challenges for SON – maintaining global network information at the level of autonomous network elements is simply illusive in large-scale and highly dynamic wireless networks. Another big challenge is the network-wide optimization of strongly interdependent network elements, with the goal of improving the efficiency of total algorithmic machinery on the network level. It is worth noting that in the telecommunication sector, environment samples corresponding to different network configurations are expensive, and online learning should have a minimum cost of affecting network service performance during training. Thus, to deliver SON solution for the 5G networks, we need to answer the following two questions:
\begin{enumerate}
    \item What information should be communicated among the network elements to enable the cooperation towards the global consensus?
    \item How to achieve consensus to improve the global network performance with high sample efficiency?
\end{enumerate}

Many works proposed reinforcement learning-based solutions for various SON use cases, as well as the coordination between the SON functions \cite{amiri2019reinforcement,mwanje2016cognitive,munoz2015load}. However, in these works, the selection of the network state information and the optimization of the learning function were considered as two independent processes. Expert knowledge is exploited to select the features and use them as the network state information, which may cause either insufficient information thus poor optimization performance, or too much redundant information thus high complexity of the learning model. 

The task-oriented communication system design can be leveraged to jointly optimize the information exaction and control optimization problems. Let us take the SON function Mobility Load Balancing (MLB) as an example. MLB is a function where cells suffering congestion can transfer load to other cells which have spare resources, by adjusting their handover (HO) control parameters (for details of HO parameters refer to \cite{lobinger2011coordinating}). Given a set of cell sites (hereafter referred to as cells) $\Ks =\{1, \ldots, K\}$, each cell can configure its HO control parameters $\vp_k\in \R^N$ and obtain a partial observation $\vo_k\in \R^M$ of the global network state $\vs\in\Ss$, where the entropy yields $H(\vo_1, \ldots, \vo_K)= H(\vs)$ and $H(\vo_k)<H(\vs)$ for $k\in\Ks$. Let $\vp:=[\vp_1, \ldots, \vp_K]$ and $\vo:=[\vo_1, \ldots, \vo_K]$ denotes the collections of HO control parameters and observations in the multi-cell network system respectively. The objective is to minimize the global cost function $\Js(\vs, \vp)$ with the information contained in the observations $\vo$. It is obvious that to learn a centralized model that takes all actions and observations $[\vp; \vo]\in\R^{(NM)^K}$ into account will lead to an extremely high model complexity. 

To reduce the computational complexity, a task-oriented communication design can be considered as shown in Fig. \ref{fig:SON_Arch}. Such design enables distributed execution of the joint training of the local communication and computing polices $\pi_k^{(c, a)}$, $k\in\Ks$. At time slot $t$, each cell observes a partial information $\vo_k(t)$ from the environment, with the policy $\pi_k^{(c, a)}(t)$, it derives an encoded message $\vc_k(t)\in\Cs_k$ which extracts the information of the local observation, and sends it to other cells via inter-cell communication channel (e.g., the X2 interface in 5G networks). After receiving the messages from other cells $\left\{\tilde{\vc}_l: l\in\Ks\setminus\{k\}\right\}$ (note that with lossless channel we may have $\tilde{\vc}_k = \vc_k$), the local policy $\pi_k^{(c, a)}(t)$ also decides the new configuration of the HO parameters $\vp(t+1)$. On the other hand, to evaluate the global performance and compute the reward for all cells, each cell sends its observation to the core network (we assume lossless channel between the cells and the core network since they usually communicate with wired connection), and the core network who defines the task computes the common reward $r(t)$ based on the received observations, and sends it to the cells as the feedback of the current state $\vs(t)$ and joint actions $\vp(t)$. Each cell learns a joint policy $\pi_k^{(c, a)}(t):\R^M\times\Pi_{l\in\Ks\setminus\{k\}}\Cs_l\to \Cs_k\times\R^N$ that maps the local observation $\vo_k$ and received messages $\{\vc_l:l\in\Ks\setminus\{k\}\}$ to a tuple of local encoded message $\vc_k$ and local control parameters $\vp_k$. In this way, the model in each cell has a input space with the cardinality $M\prod_{l\in\Ks\setminus\{k\}}|\Cs_l|$, which is dramatically smaller than the input space cardinality $(NM)^K$ of the aforementioned centralized training based on full observations and actions $(\vo, \vp)$.

   \begin{figure}[t]
          \centering
              \includegraphics[width=\columnwidth]{SON_Arch.pdf}
          \caption{Task-oriented communication design for mobility load balancing problem in 5G SON.}
          \label{fig:SON_Arch}
    \end{figure}

==> NotationsAndDefinitions.tex <==
\subsection{Notations and Definitions}\label{subsec:Definition}
% 1. here add the notations
% 2. definitions of centralized and distributed task-based communication problems
To introduce a general class of the task-oriented communication problems, let us consider a multi-agent system with a set of the agents $\Ns:={1, \ldots, N}$ with state $\vs:=[\vs_1, \ldots, \vs_N]\in \Ss$ and computing action $\va \in \As$. Note that the computing action can be considered as any kind of actions or outputs to achieve the desired task, which does not limit itself to control actions (e.g., the control parameters to be optimized) or learning functions (e.g., the estimator of a target output). Moreover, it could be a global decision, or, a collection of the agent-specific actions $\va:= [\va_1, \ldots, \va_N]$. Assume each agent $i\in\Ns$ has a partial observation of the system $\vo_i$ with $H(\vo_i)\leq H(\vs)$, where $H(\cdot)$ denotes the information entropy. Let all local observations be collected in a vector $\vo:=[\vo_1, \ldots, \vo_N]$, and we assume $H(\vo)\leq H(\vs)$.

The objective of the multi-agent system is to jointly complete a task $T(\vs(\cdot), \va(\cdot))$, where $\vs(\cdot)$ and $\va(\cdot)$ denote the sequence of states and computing actions over time, respectively. Let the task $T(\vs(\cdot), \va(\cdot))=1$ if the task is successfully completed and $0$ otherwise. We could consider various definitions of the task, e.g., maximizing a global objective function $V(\vs(\cdot), \va(\cdot))$ or learning a predictive function $f(\vs(\cdot), \va(\cdot))$, with or without constraints.

\begin{definition}[Centralized Task-Oriented Communication Problem] The centralized task-oriented communication problem aims at jointly optimizing the \textbf{coding policy} and the \textbf{computing policy}  to complete a global task, defined as follows.
\begin{itemize}
\item {\bf Coding policy}: Let $\pi^{(\C)}:\Os\to\Cs$ denote the coding policy to obtain a collection of encoded messages in the agents $\vc:=[\vc_1, \ldots, \vc_N]$ as the information extracted from the complete observation $\vo$ with $H(\vc)\leq H(\vo)$\footnote{The entropy $H(\vc)$ can be smaller than $H(\vo)$ because we may not need the complete information of the observation to complete the task.}. We have $\vc\in\Cs$ and $\vc_i\in \Cs_i$ for each $i\in\Ns$, and $\Cs:=\Pi_{i\in\Ns}\Cs_i$.
\item {\bf Communication constraints}: Consider the communication channels between each agent $i\in\Ns$ and the central coordinator $\phi_i:\Cs_i\to\Css_i:\vc_i\mapsto\vcs_i$, where $\vcs_i\in\Css_i$ denotes the received massage from agent $i$ in the coordinator. For any discrete memory-less channel, the information channel capacity can be subjected to additional constraint $\sup_{P_{C_i}(\vc_i)}I(C_i; C_i')\leq C^{(\max)}_i$.
\item {\bf Computing policy}: Let $\pi^{(\A)}:\Css\to\As$ denote the computing policy that makes a computing decision $\va$ based on the received message $\vcs$.
\item {\bf Task-oriented objective}: The task-oriented communication problem is to jointly find $\left(\hat{\pi}^{(\C)}, \hat{\pi}^{(\A)}\right)$ such that $T_{\hat{\pi}^{(\C)}, \hat{\pi}^{(\A)}}(\vs(\cdot), \va(\cdot))=1$.
\end{itemize}
\label{def:cenTBCP}
\end{definition}

% 
\begin{definition}[Distributed Task-Oriented Communication Problem] The distributed task-oriented communication problem aims at jointly optimizing the  \textbf{local coding policies} and the \textbf{local computing policies} to complete a global task, as defined below.
\begin{itemize}
\item {\bf Local coding policy}: Let $\pi^{(\C)}_i:\Os_i\to\Cs_i$  denote the local coding policy to extract an encoded messages $\vc_i$ from $\vo_i$ in each agent $i\in\Ns$. 
\item {\bf Communication constraints}: The communication channel from each agent $i\in \Ns$ to any agent $j\in \Ns\setminus\{i\}$ is denoted by $\psi_{i,j}:\Cs_i\to\Css_i: \vc_i\mapsto \vcs_{i,j}$, where $\vcs_{i,j}$ is a received copy of the sent message $\vc_i$ in agent $j$. The channel can be subjected to the capacity constraint $\sup_{P_{C_i}(\vc_i)}I(C_i; C_{i, j}')\leq C^{(\max)}_{i,j}$.   
\item {\bf Local computing policy}: Let $\pi_i^{(\A)}:\Cs_i\times\Pi_{j\in\Ns\setminus\{i\}}\Css_j\to\As_i$ denote the local computing policy that makes local decisions $\va_i, i\in\Ns$ based on the local encoded message $\vcs_i$ and the received messages $\left\{\vcs_{j, i}\right\}_{j\in\Ns\setminus\{i\}}$. Since there is no communication cost to obtain the local state in agent $i$, instead of $\vcs_i$, agent $i$ can directly utilize the original state $\vs_i$. Thus, without loss of generality, we can also define the local decision policy $\pi_i^{(\A)}:\Ss_i\times\Pi_{j\in\Ns\setminus\{i\}}\Css_j\to\As_i$.
\item {\bf Task-oriented objective}: The distributed task-oriented communication problem is to find $\left\{\left(\hat{\pi}_i^{(\C)}, \hat{\pi}_i^{(\A)}\right): \forall i\in\Ns\right\}$ such that $T_{\hat{\pi}_1^{(\C)}, \hat{\pi}_1^{(\A)}, \ldots,\hat{\pi}_N^{(\C)}, \hat{\pi}_N^{(\A)} }(\vs(\cdot), \va(\cdot))=1$.
\end{itemize}
\label{def:distTBCP}
\end{definition}

\begin{remark}
Compared against the conventional optimization problem that searches for an optimal decision policy $\pi^{\ast}:\Ss\to\As$ depending on the complete state space, the task-oriented communication scheme has the advantages of two fold: 1) \textbf{reduce the communication cost} because the entropy of the sent information yields $ H(\vc)\leq H(\vs)$, and 2) \textbf{reduce the complexity of the function to optimize the decision process}, because with $H(\vcs)\leq H(\vs)$ the input space for the learning function can be reduced. 
\end{remark}

\QL{Here I tried to generalize the definition of coding and decision policies such that they are not limited to any specific coding scheme or control/learning action. 
The \lq\lq coding policy" is just defined as a projection from the observation to a message, it is not limited to source coding or/and channel coding, it is rather an end-to-end task-oriented coding that extract and code the task-oriented information from the observations that is relevant to complete the final task. 
Also, the \lq\lq decision policy" defined here is not limited to any optimization actions or learning functions, e.g., it could be the centralized or distributed task-oriented decoder, anomaly detector, scheduling, routing, power control, or any regression/prediction/optimization actions.}

\QL{If you would like to keep these definitions, I could also add two figures for Def. 1 and 2 later. But please feel free to remove the subsection if it does not fit your definition of the task-oriented problems.}

==> TOCD review_arxiv/Application_OTA.tex <==
%\todoQL{Add an application in network level optimization in 5G/6G.}

%\QL{We may add a subsection of Over-The-Air (OTA) Computation which lies in the intersection of information theory and communication theory. This is a hot topic in communications community that takes into account the underlying task, such as computing a function, directly at the physical layer, by exploit the superposition property of the wireless channel. It allows an efficient function computation over the “air”. Here you may consider the pre-processing of the information as the \lq\lq coding policy", and the post-processing to the final desired function directly as the "action policy". References: \cite{liu2020over,cao2020optimized, frey2020over}} 

\subsection{Over-The-Air Computation in Smart Manufacturing Plants} \label{subsec:AirComp}
In IoT networks, massive amounts of data are generated, collected, and leveraged to help complete a predefined task. For example, in smart manufacturing plants, wireless data needs to be collected from thousands of sensors. However, we are not interested in the value of each individual data source, instead, we aim to obtain the \lq\lq fusion\rq\rq \ of the information contained in all data sources, e.g., computing sums or arithmetic averages. On one hand, transferring raw measurements from a large amount of different data sources to the same data collector is not spectrum efficient, especially when the measurements can be encoded to small data packets. On the other hand, the computation of massive data in an edge device as data collector with limited computation capacity can be also challenging. 

Therefore, the technique called over-the-air computation (AirComp) has been developed to enable communication- and computation-efficient data fusion of the sensing data from large amount of the concurrent sensor transmissions. It takes into account the underlying task, such as computing a function, directly at the physical layer, by exploit the superposition property of the wireless channel. In other words, it allows an efficient target function computation over the \lq\lq air\rq\rq. 

The AirComp is defined as follows. Consider $K$ wireless sensors, each having a measurement signal $s_k\in\R$, $k\in\Ks:=\{1, \ldots, K\}$ to send. On the receiver side, we expect to derive the function of the measurements of the form 
\begin{equation}
    f(s_1, \ldots, s_k) = F\left(\sum_{k=1}^K f_k(s_k)\right)
    \label{eqn:OTA_fkn}
\end{equation}

Given the multiple access communication channel $h:\field{C}^K\to\field{C}$, AirComp aims at finding a set of \textbf{pre-processing functions} $\zeta_k:\R\to\field{C}$ and a \textbf{post-processing function} $\psi:\field{C}\to \R$ such that 
\begin{equation}
f(s_1, \ldots, s_k) = \psi\Big(h\big(\zeta_1(s_1) \ldots, \zeta_K(s_K)\big)\Big)
    \label{eqn:OTA_obj}
\end{equation}
%
The pre-processing of the measurement signal and the post-processing of the received channel output obtain directly the desired computation of the target function in \eqref{eqn:OTA_fkn} by effectively integrating the communication and the computation policies. Moreover, in this way the receiver's computational task $f(\cdot)$ defined in \eqref{eqn:OTA_fkn} of processing $K$ signals is decomposed into $K+1$ small tasks $\left\{\zeta_1(\cdot), \ldots, \zeta_K(\cdot), \psi(\cdot)\right\}$ that can be distributed among sensors and the receiver, with each of them processing only one signal. 

Without loss of generality, AirComp also falls into the class of TOCC. The task is to compute $f(s_1, \ldots, s_k)$ at the receiver (e.g., a center unit) side. The problem defined above can be aligned with Definition \ref{def:TOCC} by simply integrating the computing policy into the communication policy, i.e., the encoding (pre-processing) and decoding (post-processing) policies included in the communication policy already provide the direct action to compute the desired target function as shown in Fig. \ref{fig:OTA}.  

   \begin{figure}[t]
          \centering
              \includegraphics[width=\columnwidth]{OTA.pdf}
          \caption{Over-the-air computation in smart manufacturing plants aligned with the task-oriented communication system design}
          \label{fig:OTA}
    \end{figure}

The authors of \cite{liu2020over} derived theoretical bounds on the mean squared error for a certain AirComp function (sum of the signals) computation in a fast-fading scenario with Channel State Information (CSI) available at the transmitter.  In \cite{dong2020blind}, the AirComp problem is tackled without the explicit knowledge of channel information but under the assumption of slow fading.  Then, in \cite{frey2020over} a AirComp scheme was proposed for distribution approximation of a larger class of functions than the previous works with theoretically proven bound over fast-fading channels that can deal with correlated fading and requires no CSI.

A popular application of AirComp computational techniques is the computation of distributed gradient descent to solve the empirical risk minimization problem for machine learning models. One example is the training of neural networks in a central mode but with distributed data reported by a large number of local agents such as sensors in the smart manufacturing plant. In \cite{amiri2020machine} the authors proposed to use AirComp computation over wireless channels to help efficiently computing distributed stochastic gradient descent in the Federated Learning (FL) paradigm. The author in \cite{yang2020federated} extended the idea to channels with fading channel information at either the transmitter or receiver side. In \cite{frey2020over} the authors shown the application of a proposed AirComp scheme to the regressor and classifiers in vertical FL.


\subsection{5G Self-Organizing Networks}\label{subsec:5GSON}
Although it has been almost a decade since the concept of Self-Organizing Networks (SONs) was introduced to the Next Generation Mobile Networks (NGMN) and 3GPP standards \cite{TS32500}, the existing SON solutions have not met the high expectation of the operators to achieve a fully self-aware cognitive network with automated configuring, monitoring, troubleshooting, and optimizing. This is because, with the emergence of new wireless devices and applications, it is expected that a large amount of measurements and signaling overhead will be generated in future networks, while partial and inaccurate network knowledge, together with the increasing complexity of envisioned wireless networks, pose one of the biggest challenges for SON – maintaining global network information at the level of autonomous network elements is simply illusive in large-scale and highly dynamic wireless networks. Another big challenge is the network-wide optimization of strongly interdependent network elements, with the goal of improving the efficiency of total algorithmic machinery on the network level. It is worth noting that in the telecommunication sector, environment samples corresponding to different network configurations are expensive, and online learning should have a minimum cost of affecting network service performance during training. Thus, to deliver SON solution for the 5G networks, we need to answer the following two questions:
\begin{enumerate}
    \item What information should be communicated among the network elements to enable the cooperation towards the global consensus?
    \item How to achieve consensus to improve the global network performance with high sample efficiency?
\end{enumerate}

Many works proposed reinforcement learning-based solutions for various SON use cases, as well as the coordination between the SON functions \cite{amiri2019reinforcement,mwanje2016cognitive,munoz2015load}. However, in these works, the selection of the network state information and the optimization of the learning function were considered as two independent processes. Expert knowledge is exploited to select the features and use them as the network state information, which may cause either insufficient information thus poor optimization performance, or too much redundant information thus high complexity of the learning model. 

The task-oriented communication system design can be leveraged to jointly optimize the information exaction and control optimization problems. Let us take the SON function Mobility Load Balancing (MLB) as an example. MLB is a function where cells suffering congestion can transfer load to other cells which have spare resources, by adjusting their handover (HO) control parameters (for details of HO parameters refer to \cite{lobinger2011coordinating}). Given a set of cell sites (hereafter referred to as cells) $\Ks =\{1, \ldots, K\}$, each cell can configure its HO control parameters $\vp_k\in \R^N$ and obtain a partial observation $\vo_k\in \R^M$ of the global network state $\vs\in\Ss$, where the entropy yields $H(\vo_1, \ldots, \vo_K)= H(\vs)$ and $H(\vo_k)<H(\vs)$ for $k\in\Ks$. Let $\vp:=[\vp_1, \ldots, \vp_K]$ and $\vo:=[\vo_1, \ldots, \vo_K]$ denotes the collections of HO control parameters and observations in the multi-cell network system respectively. The objective is to minimize the global cost function $\Js(\vs, \vp)$ with the information contained in the observations $\vo$. It is obvious that to learn a centralized model that takes all actions and observations $[\vp; \vo]\in\R^{(NM)^K}$ into account will lead to an extremely high model complexity. 

To reduce the computational complexity, a task-oriented communication design can be considered as shown in Fig. \ref{fig:SON_Arch}. Such design enables distributed execution of the joint training of the local communication and computing polices $\pi_k^{(c, a)}$, $k\in\Ks$. At time slot $t$, each cell observes a partial information $\vo_k(t)$ from the environment, with the policy $\pi_k^{(c, a)}(t)$, it derives an encoded message $\vc_k(t)\in\Cs_k$ which extracts the information of the local observation, and sends it to other cells via inter-cell communication channel (e.g., the X2 interface in 5G networks). After receiving the messages from other cells $\left\{\tilde{\vc}_l: l\in\Ks\setminus\{k\}\right\}$ (note that with lossless channel we may have $\tilde{\vc}_k = \vc_k$), the local policy $\pi_k^{(c, a)}(t)$ also decides the new configuration of the HO parameters $\vp(t+1)$. On the other hand, to evaluate the global performance and compute the reward for all cells, each cell sends its observation to the core network (we assume lossless channel between the cells and the core network since they usually communicate with wired connection), and the core network who defines the task computes the common reward $r(t)$ based on the received observations, and sends it to the cells as the feedback of the current state $\vs(t)$ and joint actions $\vp(t)$. Each cell learns a joint policy $\pi_k^{(c, a)}(t):\R^M\times\Pi_{l\in\Ks\setminus\{k\}}\Cs_l\to \Cs_k\times\R^N$ that maps the local observation $\vo_k$ and received messages $\{\vc_l:l\in\Ks\setminus\{k\}\}$ to a tuple of local encoded message $\vc_k$ and local control parameters $\vp_k$. In this way, the model in each cell has a input space with the cardinality $M\prod_{l\in\Ks\setminus\{k\}}|\Cs_l|$, which is dramatically smaller than the input space cardinality $(NM)^K$ of the aforementioned centralized training based on full observations and actions $(\vo, \vp)$.

   \begin{figure}[t]
          \centering
              \includegraphics[width=\columnwidth]{SON_Arch.pdf}
          \caption{Task-oriented communication design for mobility load balancing problem in 5G SON.}
          \label{fig:SON_Arch}
    \end{figure}

==> TOCD review_arxiv/NotationsAndDefinitions.tex <==
\subsection{Notations and Definitions}\label{subsec:Definition}
% 1. here add the notations
% 2. definitions of centralized and distributed task-based communication problems
To introduce a general class of the task-oriented communication problems, let us consider a multi-agent system with a set of the agents $\Ns:={1, \ldots, N}$ with state $\vs:=[\vs_1, \ldots, \vs_N]\in \Ss$ and computing action $\va \in \As$. Note that the computing action can be considered as any kind of actions or outputs to achieve the desired task, which does not limit itself to control actions (e.g., the control parameters to be optimized) or learning functions (e.g., the estimator of a target output). Moreover, it could be a global decision, or, a collection of the agent-specific actions $\va:= [\va_1, \ldots, \va_N]$. Assume each agent $i\in\Ns$ has a partial observation of the system $\vo_i$ with $H(\vo_i)\leq H(\vs)$, where $H(\cdot)$ denotes the information entropy. Let all local observations be collected in a vector $\vo:=[\vo_1, \ldots, \vo_N]$, and we assume $H(\vo)\leq H(\vs)$.

The objective of the multi-agent system is to jointly complete a task $T(\vs(\cdot), \va(\cdot))$, where $\vs(\cdot)$ and $\va(\cdot)$ denote the sequence of states and computing actions over time, respectively. Let the task $T(\vs(\cdot), \va(\cdot))=1$ if the task is successfully completed and $0$ otherwise. We could consider various definitions of the task, e.g., maximizing a global objective function $V(\vs(\cdot), \va(\cdot))$ or learning a predictive function $f(\vs(\cdot), \va(\cdot))$, with or without constraints.

\begin{definition}[Centralized Task-Oriented Communication Problem] The centralized task-oriented communication problem aims at jointly optimizing the \textbf{coding policy} and the \textbf{computing policy}  to complete a global task, defined as follows.
\begin{itemize}
\item {\bf Coding policy}: Let $\pi^{(\C)}:\Os\to\Cs$ denote the coding policy to obtain a collection of encoded messages in the agents $\vc:=[\vc_1, \ldots, \vc_N]$ as the information extracted from the complete observation $\vo$ with $H(\vc)\leq H(\vo)$\footnote{The entropy $H(\vc)$ can be smaller than $H(\vo)$ because we may not need the complete information of the observation to complete the task.}. We have $\vc\in\Cs$ and $\vc_i\in \Cs_i$ for each $i\in\Ns$, and $\Cs:=\Pi_{i\in\Ns}\Cs_i$.
\item {\bf Communication constraints}: Consider the communication channels between each agent $i\in\Ns$ and the central coordinator $\phi_i:\Cs_i\to\Css_i:\vc_i\mapsto\vcs_i$, where $\vcs_i\in\Css_i$ denotes the received massage from agent $i$ in the coordinator. For any discrete memory-less channel, the information channel capacity can be subjected to additional constraint $\sup_{P_{C_i}(\vc_i)}I(C_i; C_i')\leq C^{(\max)}_i$.
\item {\bf Computing policy}: Let $\pi^{(\A)}:\Css\to\As$ denote the computing policy that makes a computing decision $\va$ based on the received message $\vcs$.
\item {\bf Task-oriented objective}: The task-oriented communication problem is to jointly find $\left(\hat{\pi}^{(\C)}, \hat{\pi}^{(\A)}\right)$ such that $T_{\hat{\pi}^{(\C)}, \hat{\pi}^{(\A)}}(\vs(\cdot), \va(\cdot))=1$.
\end{itemize}
\label{def:cenTBCP}
\end{definition}

% 
\begin{definition}[Distributed Task-Oriented Communication Problem] The distributed task-oriented communication problem aims at jointly optimizing the  \textbf{local coding policies} and the \textbf{local computing policies} to complete a global task, as defined below.
\begin{itemize}
\item {\bf Local coding policy}: Let $\pi^{(\C)}_i:\Os_i\to\Cs_i$  denote the local coding policy to extract an encoded messages $\vc_i$ from $\vo_i$ in each agent $i\in\Ns$. 
\item {\bf Communication constraints}: The communication channel from each agent $i\in \Ns$ to any agent $j\in \Ns\setminus\{i\}$ is denoted by $\psi_{i,j}:\Cs_i\to\Css_i: \vc_i\mapsto \vcs_{i,j}$, where $\vcs_{i,j}$ is a received copy of the sent message $\vc_i$ in agent $j$. The channel can be subjected to the capacity constraint $\sup_{P_{C_i}(\vc_i)}I(C_i; C_{i, j}')\leq C^{(\max)}_{i,j}$.   
\item {\bf Local computing policy}: Let $\pi_i^{(\A)}:\Cs_i\times\Pi_{j\in\Ns\setminus\{i\}}\Css_j\to\As_i$ denote the local computing policy that makes local decisions $\va_i, i\in\Ns$ based on the local encoded message $\vcs_i$ and the received messages $\left\{\vcs_{j, i}\right\}_{j\in\Ns\setminus\{i\}}$. Since there is no communication cost to obtain the local state in agent $i$, instead of $\vcs_i$, agent $i$ can directly utilize the original state $\vs_i$. Thus, without loss of generality, we can also define the local decision policy $\pi_i^{(\A)}:\Ss_i\times\Pi_{j\in\Ns\setminus\{i\}}\Css_j\to\As_i$.
\item {\bf Task-oriented objective}: The distributed task-oriented communication problem is to find $\left\{\left(\hat{\pi}_i^{(\C)}, \hat{\pi}_i^{(\A)}\right): \forall i\in\Ns\right\}$ such that $T_{\hat{\pi}_1^{(\C)}, \hat{\pi}_1^{(\A)}, \ldots,\hat{\pi}_N^{(\C)}, \hat{\pi}_N^{(\A)} }(\vs(\cdot), \va(\cdot))=1$.
\end{itemize}
\label{def:distTBCP}
\end{definition}

\begin{remark}
Compared against the conventional optimization problem that searches for an optimal decision policy $\pi^{\ast}:\Ss\to\As$ depending on the complete state space, the task-oriented communication scheme has the advantages of two fold: 1) \textbf{reduce the communication cost} because the entropy of the sent information yields $ H(\vc)\leq H(\vs)$, and 2) \textbf{reduce the complexity of the function to optimize the decision process}, because with $H(\vcs)\leq H(\vs)$ the input space for the learning function can be reduced. 
\end{remark}

\QL{Here I tried to generalize the definition of coding and decision policies such that they are not limited to any specific coding scheme or control/learning action. 
The \lq\lq coding policy" is just defined as a projection from the observation to a message, it is not limited to source coding or/and channel coding, it is rather an end-to-end task-oriented coding that extract and code the task-oriented information from the observations that is relevant to complete the final task. 
Also, the \lq\lq decision policy" defined here is not limited to any optimization actions or learning functions, e.g., it could be the centralized or distributed task-oriented decoder, anomaly detector, scheduling, routing, power control, or any regression/prediction/optimization actions.}

\QL{If you would like to keep these definitions, I could also add two figures for Def. 1 and 2 later. But please feel free to remove the subsection if it does not fit your definition of the task-oriented problems.}

==> TOCD review_arxiv/macros_QL.tex <==
\usepackage[normalem]{ulem}
\newcommand{\QL}[1]{\textbf{\textcolor{blue}{(QL: #1)}}}
\newcommand{\todoQL}[1]{\textbf{\textcolor{red}{(Todo QL: #1)}}}
\newcommand{\inQL}[1]{\textcolor{blue}{#1}}
\newcommand{\rmQL}[1]{\textcolor{red}{\sout{#1}}} 
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\menge}[1]{\mathcal{#1}}
\newcommand{\ma}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\ve}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\vo}{\ve{o}}
\newcommand{\vs}{\ve{s}}
\newcommand{\va}{\ve{a}}
\newcommand{\vh}{\ve{h}}
\newcommand{\vp}{\ve{p}}
\newcommand{\vc}{\ve{c}}
\newcommand{\vcs}{\ve{c}'}
\newcommand{\Ss}{\menge{S}}
\newcommand{\As}{\menge{A}}
\newcommand{\Js}{\menge{J}}
\newcommand{\Os}{\menge{O}}
\newcommand{\Cs}{\menge{C}}
\newcommand{\Ps}{\menge{P}}
\newcommand{\Ks}{\menge{K}}
\newcommand{\Css}{\menge{C}'}
\newcommand{\Ns}{\menge{N}}
\newcommand{\R}{\field{R}}
%\newcommand{\C}{\field{C}}
\DeclareMathOperator*\argmin{arg \, min}		% arg min
\DeclareMathOperator*\maximize{maximize}
%\DeclareMathOperator*\sup{sup}
%\DeclareMathOperator*\max{max}
\DeclareMathOperator*\subject{subject \ to}	
\DeclareMathOperator*\I{I}
\DeclareMathOperator*\C{C}
\DeclareMathOperator*\D{D}
\DeclareMathOperator*\A{A}
\DeclareMathOperator*\T{T}

